BMS Symmetries of Gravitational Scattering

After motivating the relevance of the Bondi-Metzner-Sachs (BMS) group over the last decades, we review how concepts such as Penrose diagrams and the covariant phase space formalism can be used to understand the asymptotic structure of asymptotically flat spacetimes (AFS). We then explicitly construct the asymptotic symmetry group of AFS in $3+1$ dimensions, the BMS group. Next, we apply this knowledge to the usual far-field scattering problem in general relativity, which leads to the unravelling of the intrinsic features of gravity in the infrared. In particular, we work out the connections between asymptotic symmetries, soft theorems in quantum field theories and gravitational memory effects. We restrict to the study of this infrared triangle through the lens of supertranslations here, but the analogous features that can be found in the case of superrotations or for other gauge theories are also motivated at the end of our discussion. We conclude with an overview of the implications of the infrared triangle of gravity for the formulation of an approach to quantum gravity through holography, as well as a brief discussion of its potential in tackling the black hole information paradox.

==> 0B-disclaimer.tex <==
\thispagestyle{empty}

\vspace*{\fill}
\begin{center}
\begin{minipage}{0.5\textwidth} 
    \begin{flushleft} 
    \large
    \textit{`` Nothing in physics seems so hopeful to as the idea that it is possible for a theory to have a high degree of symmetry was hidden from us in everyday life. The physicist's task is to find this deeper symmetry. ''}
    \end{flushleft}
    \begin{flushright}
        \large -- \textit{Steven Weinberg. \\ “The Forces of Nature.” (1976)}
    \end{flushright}
\end{minipage}
\end{center}
\vspace*{\fill}
